In-context Learning and Gradient Descent Revisited

In-context learning (ICL) has shown impressive results in few-shot learning tasks, yet its underlying mechanism is still not fully understood. A recent line of work suggests that ICL performs gradient descent (GD)-based optimization implicitly. While appealing, much of the research focuses on simplified settings, where the parameters of a shallow model are optimized. In this work, we revisit evidence for ICL-GD correspondence on realistic NLP tasks and models. We find gaps in evaluation, both in terms of problematic metrics and insufficient baselines. We show that surprisingly, even untrained models achieve comparable ICL-GD similarity scores despite not exhibiting ICL. Next, we explore a major discrepancy in the flow of information throughout the model between ICL and GD, which we term Layer Causality. We propose a simple GD-based optimization procedure that respects layer causality, and show it improves similarity scores significantly.

==> resources/images/prediction_alignment.tex <==
% \begin{figure*}[h!]
%   \centering
%   \includegraphics[width=0.98\linewidth,height=6cm]{resources/images/prediction_alignment.png}
%   \caption{
%     Partition of prediction changes with regards to the zero-shot setting induced by ICL and FT.
%     For each task, we evaluate both methods on the same validation set.
%     Correct changes are examples that are misclassified in the ZSL setting and are correctly classified following the prediction update.
%     incorrect changes are examples whose prediction is changed from the ZSL setting into an incorrect label.
%   }
%   \label{fig:prediction_alignment}
% \end{figure*}

==> resources/tables/acc_jaccard.tex <==
\begin{table*}[ht!]
  \centering
  \setlength{\tabcolsep}{7pt}
  \begin{tabular}{l | c c c c c c}
  \toprule
  & \textbf{CB} & \textbf{SST2} & \textbf{SST5} & \textbf{Subj} & \textbf{MR} & \textbf{AGNews} \\ 
  \midrule
   ZSL Accuracy & 37.5 & 70.5 & 39.3 & 72.6 & 65.9 & 46.2 \\
   FT Accuracy & 57.1 & 74 & 39.4 & 77.8 & 72.6 & 66.7 \\
   ICL Accuracy & 50 & 92.7 & 45.0 & 90.0 & 89.1 & 79.2 \\
  \midrule
  Jaccard Index (\%)           & 80.0 & 16.4 & 3.4 & 36.2 & 34.0 & 48.0 \\
  Jaccard - Correct (\%) & 91.7 & 19.8 & 3.2 & 48.0 & 40.2 & 63.5 \\
  Jaccard - Incorrect (\%) & 66.7 & 1.8 & 3.5 & 10.2 & 17.7 & 19.2 \\
  \end{tabular}
  \caption{Validation accuracy and Jaccard Index for ZSL, finetuning, and ICL settings on all six classification datasets.}
  \label{tab:acc_jaccard}
\end{table*}

==> resources/tables/layer_causal_clipped.tex <==
\begin{table}[H]
	\centering
	\setlength{\tabcolsep}{7pt}
		\begin{tabular}{l | c}
		\toprule
		& \textbf{Subj} \\
		\midrule
		 SimAUO (GD)     & 0.1932 \\
		 SimAUO (LCGD Clipped)   & \textbf{0.3480}  \\
		\midrule
		 SimAM (ZSL)                     & 0.3786 \\
		 SimAM (GD)             & \textbf{0.4870} \\
		 SimAM (LCGD Clipped)           & 0.4227 \\
		
		\end{tabular}
	\caption{
		% Left shows the results for the per-layer training process. Middle shows the results for the per-layer training process with gradient norm clipping. Right shows the results for the standard fine-tuning process.
		Comparison of layer causal GD with gradient clipping.
		These results show that even arbitrary clipping may resolve the drop in SimAM shown in Table \ref{tab:layer_causal}.
	}
	\label{tab:per_layer_clipping_metrics}
\end{table}

==> resources/tables/linearized_gd.tex <==
\begin{table*}
	\centering
  \setlength{\tabcolsep}{7pt}
	\begin{tabular}{l | c c c c c }
    \toprule
    & SST2   & SST5   & MR     & Subj  & Average \\
		\midrule
    SimAOU (Random)   & 0.001  & 0.002  & 0.001  & 0.002 & 0.002          \\
		SimAOU (FT)       & 0.1091 & \textbf{0.113}  & \textbf{0.219}  & \textbf{0.193} & \textbf{0.158} \\
		SimAOU (FT Lin)   & \textbf{0.122}  & 0.0789 & 0.171  & 0.148 & 0.130          \\
    \midrule
    SimAM (Before FT)     & 0.5547 & 0.3914 & 0.398 & 0.378 & 0.430          \\
    SimAM (After FT)      & \textbf{0.585}  & \textbf{0.404}  & \textbf{0.498} & \textbf{0.487} & \textbf{0.493} \\
    SimAM (After FT Lin)  & 0.573  & 0.403  & 0.448 & 0.449 & 0.468          \\
  \end{tabular}

	\caption{
    SimAOU and SimAM comparison of standard FT and FT using the linear approximation of the model.	 		
  }
	\label{tabel:lin_results}
\end{table*}
